Analysis of Stochastic Processes through Replay Buffers

Replay buffers are a key component in many reinforcement learning schemes. Yet, their theoretical properties are not fully understood. In this paper we analyze a system where a stochastic process X is pushed into a replay buffer and then randomly sampled to generate a stochastic process Y from the replay buffer. We provide an analysis of the properties of the sampled process such as stationarity, Markovity and autocorrelation in terms of the properties of the original process. Our theoretical analysis sheds light on why replay buffer may be a good de-correlator. Our analysis provides theoretical tools for proving the convergence of replay buffer based algorithms which are prevalent in reinforcement learning schemes.

==> Experiments.tex <==
\section{Experiments} \label{section:experiments}

In this section we demonstrate our main theoretical results. The environment we investigate is an MRP (Markov reward process) as shown in Figure XXXX. There are total of 30 states divided into 3 blocks, 10 states in a block. The connectivity inside each block is high, however, the probability of moving from one block to another, $p_{\text{out}}$, is low. $p_{\text{out}}$ will determine the mixing time of the Markov chain: as $p_{\text{out}}$ decreases, the mixing time increases. Each block has different reward: $\{0, 1, 2\}$. We compare between two reward estimations methods: (1) Online - the estimate is updated at every step according to the last reward observation; %(2) Online-last $\NBATCH$ - the estimate is updated at every step according to the last $\NBATCH$ reward observations; 
(2) RB - the estimate is updated at every step according to a random batch of $\NBATCH$ samples from a RB with size $N$. 

We relate these estimation types to the stochastic process we defined in Section \ref{sec:RB_properties}.

\begin{align*}
    W_t & = r_t - \eta_{t-1} \\
    Z_t & = \frac{1}{\NBATCH} \sum_{t_i \in \mathcal{C}} r_{t_i}
\end{align*}
where $\mathcal{C}$ is a set of random $\NBATCH$ time samples from $RB_t$ with size $N$. 
\begin{align*}
    \eta^{\text{online}}_t &  = \eta_{t-1} + \frac{1}{t} W_t \\
    %\eta^{\text{online-last-\NBATCH}}_t & = \eta_{t-1} + \frac{1}{t} \left( \frac{1}{\NBATCH} \sum_{i=t-\NBATCH}^t r_i - \eta_{t-1} \right) \\
    \eta^{\text{RB}}_t &  = \eta_{t-1} + \frac{1}{t} Z_t
\end{align*}
In the following experiments we are interested in:
\begin{enumerate}
    \item How do the RB size $N$ and the batch size $\NBATCH$ affect the learning process, and if these sizes are connected the the MRP property of mixing time, described as $p_{\text{out}}$.
    \item How does the RB affect variance reduction.
\end{enumerate}

%%% experiment images:
\begin{figure}[t]
\centerline{\includegraphics[width=0.9\columnwidth]{pictures/diff_N.png}}
\caption{Different N values}
\label{fig:diff_N}
\end{figure}

In Figure \ref{fig:diff_N} we fixed $p_{\text{out}}$ and compared the RB estimator between different RB size $N$ values (subplots (a)-(d) in Figure \ref{fig:diff_N}). For each value of $N$, we plotted several values of $\NBATCH$, such that $\NBATCH \le N$. We can see that when $N$ is fixed, increasing $\NBATCH$ does not affects too much on the RB estimator smoothness. However, increasing $N$ do affect the RB estimator smoothness. 

\begin{figure}[t]
\centerline{\includegraphics[width=0.9\columnwidth]{pictures/diff_K.png}}
\caption{Different K values}
\label{fig:diff_K}
\end{figure}

In Figure \ref{fig:diff_K} we fixed $p_{\text{out}}$ and compared the RB estimator between different $\NBATCH$ values (subplots (a)-(d) in Figure \ref{fig:diff_K}). For each value of $\NBATCH$, we plotted several values of $N$, such that $\NBATCH \le N$. We can see that when $\NBATCH$ is fixed, increasing $N$ results a smoother RB estimator. 

\begin{figure}[t]
\centerline{\includegraphics[width=0.9\columnwidth]{pictures/p_out.png}}
\caption{Different $p_{\text{out}}$ values}
\label{fig:diff_p}
\end{figure}

In Figure \ref{fig:diff_p} we fixed the batch size $\NBATCH$ and compared the online and the RB estimators in different values of $p_{\text{out}}$ and different values of RB size $N$. Recall that as $p_{\text{out}}$ decreases, the Markov chain mixing time increases, meaning it will take longer to the Markov chain to converge to its stationary distribution. We can see that as $p_{\text{out}}$ decreases (subplots (a)-(d) in Figure \ref{fig:diff_p} ), the difference between the online and RB estimators become more significant. The RB estimator with larger size $N$ converges more smoothly, while the online estimator is noisier. 

\begin{figure}[t]
\centerline{\includegraphics[width=0.9\columnwidth]{pictures/variance.png}}
\caption{Variance}
\label{fig:variance}
\end{figure}

In Figure \ref{fig:variance} we compare the variance between the online estimator and the RB estimators for different values of $N$ and $\NBATCH$. In Figure \ref{fig:variance} (a) - (c) we can see that for a fixed values of batch size $\NBATCH$, the variance decreases as the size of the RB $N$ increases. In Figure \ref{fig:variance} (d) - (f)  we can see that for a fixed value of RB size $N$, the variance decreases as the batch size $\NBATCH$ increases. In addition the variance of the RB estimator in all the experiments is always kept smaller than the variance of the online estimator at the first stage of learning. As learning progresses, both variances tend to 0. 

% Note that since our online estimator uses the last $\NBATCH$ observations for the reward estimation, it also affected by the size of $\NBATCH$ and also its variance decreases as $\NBATCH$ increases. 




==> sampling_methods.tex <==
a 
% In this section we focus on two common sampling methods in RL to choose a minibatch pf samples from a RB:
%\begin{definition}
%$\PS^{N,\NBATCH}$ is a probability measure for sampling $\NBATCH$ samples out of $N$ samples, according to some prioritizing sampling method. 
%\end{definition}

%\begin{enumerate}
%    \item $\PB^{N,\NBATCH}(\mathbb{I}) = %\frac{1}{\binom{N}{\NBATCH}} \ \forall \mathbb{I} \in \mathbb{C}_{N,K}$. 
%    \item $\PPER^{N,\NBATCH}(\mathbb{I}) = \prod_{i=1}^\NBATCH \frac{p_i}{\sum_{j=1}^N p_j}$ \cite{schaul2015prioritized}. \sd{define it more precisely, according to the decreasing number of samples}
%\end{enumerate}
